Vision Language Model is NOT All You Need: Augmentation Strategies for Molecule Language Models

Recently, there has been a growing interest among researchers in understanding molecules and their textual descriptions through molecule language models (MoLM). However, despite some early promising developments, the advancement of MoLM still trails significantly behind that of vision language models (VLM). This is because unique challenges exist apart from VLM in the field of MoLM due to 1) a limited amount of molecule-text paired data and 2) missing expertise that occurred due to the specialized areas of focus among the experts. To this end, we propose AMOLE, which 1) augments molecule-text pairs with structural similarity preserving loss, and 2) transfers the expertise between the molecules. Specifically, AMOLE enriches molecule-text pairs by sharing descriptions among structurally similar molecules with a novel structural similarity preserving loss. Moreover, we propose an expertise reconstruction loss to transfer knowledge from molecules that have extensive expertise to those with less expertise. Extensive experiments on various downstream tasks demonstrate the superiority of AMOLE in comprehending molecules and their descriptions, highlighting its potential for application in real-world drug discovery. The source code for AMOLE is available at https://github.com/Namkyeong/AMOLE.

==> sections/ethics.tex <==
This paper aims to advance the scientific domain by applying machine learning techniques. 
Our research is grounded in a broad spectrum of scientific literature, which has been accumulated through a long history of molecular science, underscoring the need for enhanced collaboration with diverse experts in the domain for the continued advancement of AI and scientific fields. 
Additionally, while our work has the potential for wide societal impacts, we do not believe any specific ethical impact requires particular emphasis in this discussion.

==> sections/limitations.tex <==
While this paper suggests augmenting the molecule-text pairs by sharing descriptions among similar molecules, this method does not increase the total number of descriptions. 
A potential strategy to augment the absolute number of descriptions involves generating new descriptions based on the recent achievements of decoder-only models like GPT, and adapting the style of one expert to another. 
Although this presents a viable direction, unlike the domain of VLM, generating descriptions necessitates expert knowledge, introducing an additional challenge during the generation process.
